Few-Shot Adaptation of Generative Adversarial Networks

Generative Adversarial Networks (GANs) have shown remarkable performance in image synthesis tasks, but typically require a large number of training samples to achieve high-quality synthesis. This paper proposes a simple and effective method, Few-Shot GAN (FSGAN), for adapting GANs in few-shot settings (less than 100 images). FSGAN repurposes component analysis techniques and learns to adapt the singular values of the pre-trained weights while freezing the corresponding singular vectors. This provides a highly expressive parameter space for adaptation while constraining changes to the pretrained weights. We validate our method in a challenging few-shot setting of 5-100 images in the target domain. We show that our method has significant visual quality gains compared with existing GAN adaptation methods. We report qualitative and quantitative results showing the effectiveness of our method. We additionally highlight a problem for few-shot synthesis in the standard quantitative metric used by data-efficient image synthesis works. Code and additional results are available at http://e-271.github.io/few-shot-gan.

==> rebuttal.tex <==
We thank the reviewers for their constructive comments. We respond to the core questions below.

\review{R7, R8, R9}{\textit{"brief theoretical analysis on the proposed method..."}} 

The PCA decomposition transforms the parameters of a pre-trained model into a new space, in which the principal components represent orthogonal directions of variance and the eigenvalues represent the magnitude. 
Our method rescales the \emph{eigenvalues}, but does change the eigenvectors (direction), so the underlying distribution of parameters remains the same. 
Our experiments shows that our approach preserve natural image features from the pretrain distribution while transferring domains.
In contrast, baseline methods often produce lower-quality or overfitted images.

\review{R7}{\textit{"What kinds of domains can be well transferred?"}} 

We show in Fig. 3 of the supplementary material that our model does not perform well when transferring between distant domains such as ImageNet $\rightarrow$ Anime. 
In Fig. 6 and  Fig. 7, we show that more distant domain of FFHQ -> Rem does not fully transfer, although quality is high and attributes such as hair color, gender, and skin tone are transferred. 

\review{R7}{\textit{"Difference between the proposed method and performing affine transformation ... or modulation .. (or) scaling..."}}
% It seems that some important baselines are missing. This work proposes to fine-tune the singular value of the weights only. What is the difference between the proposed method and performing affine transformation to the weights, or modulation to the weights (like the modulation in StyleGAN2)? What if we only fine-tune the weights' scaling parameters?

We compare with SSGAN, which fine-tunes the mean and variance of channels, and we find that this transformation is limited as shown in the experimental results. 
While channel scale & shift is not equivalent to weight scale & shift, we believe weight scale \& shift may have similar limitations. We note that StyleGAN2 modulation also enables a channel-wise scale \& shift.

% \textbf{7.2} "What makes the proposed better compare with other simple baselines? What does the SVD reserve from weights?"
% The main experiments focus on discussing the visual quality of the results, and the experiments show the effectiveness of the proposed method. However, why the proposed method works is also interested. As mentioned in the above question, what makes the proposed better compare with other simple baselines?
% Few-shot transfer utilizes the learned knowledge in the original GAN model. What does the SVD reserve from weights? Is this associated with the motivation of using SVD?

% Preserving the principal components constrains the degree of transfer from the source dataset, as can be seen in the Fig 6 "Rem" example where the transferred generator produces natural human-like images but with similar attributes (hair, skin tone, age, gender) of the art "Rem" dataset. This is our motivation for using PCA, because it prevents the generator from devolving into low-quality or overfit images like the fine-tuning baselines.

% \textbf{7.3} "What kinds of domains can be well transferred?" 
% Transfer knowledge of GANs between different domains in an interesting idea. However, what kinds of domains can be well transferred? Can church models transfer to conference room models, or bedroom models, and even face models?

\review{R7}{\textit{"The effectiveness of the proposed Perceptual Gradient Sparsity should be first presented."}}

We demonstrate the effectiveness in Fig. 3 of the text. 
Early iterations starting from the pretrain English dataset interpolate smoothly and do not appear overfit. Later iterations clearly overfit to the 10-image Kannada dataset and report poor PGS. 
We will add additional ablation to the supplementary material.

% \textbf{8.1} Line132, "transform the generated sample distribution" doesn’t make sense. Line133, "during the pre-training stage": doesn’t the method use a already pre-trained network and fine-tune it?

% Thanks for pointing this out. Our meaning is that we want to preserve the diversity and quality of the pre-trained checkpoint, while transferring generated images into a new low-shot domain. We will clarify this in the revision.

% \textbf{8.2} Line134, "the underlying distribution" means which distribution?

% We mean the distribution of network parameters.

% \textbf{8.3} Line 200-201, which pre-trained checkpoint is transferred to which target dataset is not clear. For example, is the LSUN Churches pretrained checkpoint transferred to single-ID CelebA?

% This can be seen in Fig 4 and Fig 6, where the pre-trained generated image is shown under “Pretrain”. We transfer in the following settings:
% FFHQ -> CelebA single-ID
% FFHQ -> Portrait
% FFHQ -> Rem
% LSUN Churches -> Van Gogh landscapes

% \textbf{8.1} "Why statistical parameters are rescaled but the underlying distribution is unchanged?"
% Why SVD principle components of pre-trained weights on one dataset can be used on another dataset is unclear. The authors didn't give any sound reason for this. "Our method is to rescale statistical parameters without changing the underlying distribution." is hard to understand. Why statistical parameters are rescaled by the underlying distribution is unchanged? Can the pre-trained weights on the LSUN churches dataset be used on the face images? Is there any assumption required to use this method?

\review{R8}{\textit{"The SinGAN can generate images with good quality using a single image."}}

Thanks for your comment, we will clarify this point. As discussed in Section 2, 1-shot generators are a different setting, as they learn the distribution of visual elements internal to a single image. Our setting is highly diverse images domains with only a few training images, for which high-quality diverse image generation has not previously been demonstrated.

\review{R8}{\textit{"I can't see connection between the Few-short GAN images and the pretrain images."}}
%In Fig. 6, I can't see how good are the generated images from Few-short GAN. The results of SSGAN make sense because the content is like the images from the pretrain column, and the style is transferred to the target domain. I can't see connection between the Few-short GAN images and the pretrain images. 

We note that our setting is domain transfer rather than style transfer, so we do not require resemblance between pretrain and transferred images in Fig. 6. 
In the far-domain setting, the degree of domain transfer varies based on the distance between pretrain and transfer domain, so resemblance will vary.
The purpose of Fig. 6 is to highlight the quality of the Few-shot GAN far-domain transfer, and demonstrate which features of the target dataset our method learns.

\review{R8}{\textit{"Are the Few-short GAN images just some existing images in the target domain?"}}

No, the entire target dataset is shown in Fig 6, and from inspection generated images are not in the target domain.

\review{R8}{\textit{"In table 1, the proposed method doesn't outperforms other methods even under the proposed PGS metric. Under FID, the proposed method is worse than existing methods in most of the cases. In the user study (Figure 7), the proposed method is worse than existing methods in 50\% of the experiments."}}
% Performance on PGS, FID, and user study}

We do not optimize for PGS directly because it doesn't reflect quality or domain transfer, it only signals overfitting.
As discussed in Section 3, FID is not well suited to the low data setting. Also as shown in Fig 7, FID does not correlate well with human evaluations of quality.
Fig. 7 demonstrates that Few-shot GAN achieves best quality by far across all comparison datasets. Transfer results are competitive with other methods.

% {8.9} Eq (5) indicates that the input “z” to the Generator is a scaler value sampled from a 1d Gaussian. However, in all GAN papers, the latent vector “z” is a high dimensional vector. Why z is only a scaler here?

% Thanks for pointing this out. z is sampled from a multivariate Gaussian, we will change the notation this in the revision.

% {8.10} Eq. (7) is not correct. G(z) is an image. The dimension of left hand side is the image size by the latent vector size, but the dimension of the right hand side is the latent vector size.

% Thanks for pointing this out, we provide a revised equation for Fig. 7:

% {8.11} In line 191, 192, why "in the multi-mode overfitting case, high PGS indicates overfitting. In the single-mode overfitting case, a low PGS may indicate overfitting"?

% In the multi-mode overfitting the latent space gradients are either near-zero or very large, so the sparsity is high. In the single-mode overfitting case the latent space gradients will all be zero or near-zero, so the sparsity is very low (we observe near-zero).

% {8.13} The generator of Figure 2 is confusing. The way the the generator is drawn seems to me that the Generator takes an image as input and outputs a vector.

% Thanks for pointing this out. We will clarify this by removing the few-shot target dataset from this figure in the revision.

% \textbf{9.1}  
% Theoretical analysis is not presented to give a clear explanation for the proposed method. The authors did not explain the reason why they used PCA to decompose the weights, and why the proposed method can be used to tackle the multi-mode over-fitting problem. Could you please give a brief theoretical analysis on the proposed method and the experimental results?

% - We use PCA decomposition because it allows us to change the variance of the pretrained weights without changing the underlying distribution.
%- We find that constraining the parameters to the principal component coefficients prevents the multi-mode overfitting, because it limits the amount the network can change. 

\review{R9}{\textit{"...apply (PGS) as an early stopping criterion on other baseline methods?"}}
% The proposed metric is used as an early stopping criterion during the training period on the target domain. Although this helps to detect multi-mode overfitting phenomenon, is it possible to apply this metric as an early stopping criterion on other baseline methods?

Our reported results use do PGS as an early stopping criterion for baselines. We note that PGS is actually more useful for the baselines than for our PCA-based method, because the baselines have more capacity to overfit. 


% \review{R9}{The author can give a formal description on the optimization period of the introduced lambda.}

% We will include more training details in the supplementary material.

%\textbf{9.5} It it better to make each figure cited in the main paper, especially for Figure 2. It may help to make the framework easier to understand.

%Thanks for point this out, we will add these references.

\review{R9}{\textit{"Is it possible to improve the PGS metric to be a regularization term in the training period?"}}

Thanks for your suggestion, we believe this is a good direction for future research. However, we find that our PCA-based method is less prone to overfitting compared with baselines, so the regularization may not be as helpful.

\review{R9}{\textit{"Since the technical contributions are independently fold into two parts, ablation study can be given to prove the effectiveness of the proposed method."}}
% The experiment may be not sufficient. Since the technical contributions are independently fold into two parts, ablation study can be given to prove the effectiveness of the proposed method. For example, (a). baseline without PGS. (b). baseline with PGS. (c) the proposed PCA-based adaption without PGS. (d) the proposed PCA-based adaption with PGS.

Thanks for this suggestion. We will add this ablation.

%{9.7} It may be not strict to name the two settings as ‘in-domain transfer’ and ‘cross-domain transfer’ in Section 3, since the problem is natually a cross-domain problem. Maybe it’s better to use expressions like ‘short-ranger transfer’ and ‘long-range transfer’ to prevent ambiguity.

%Thanks for this suggestion, we agree that terminology is more clear.


